The impact of feature importance methods on the interpretation of defect classifiers

Classifier specific (CS) and classifier agnostic (CA) feature importance methods are widely used (often interchangeably) by prior studies to derive feature importance ranks from a defect classifier. However, different feature importance methods are likely to compute different feature importance ranks even for the same dataset and classifier. Hence such interchangeable use of feature importance methods can lead to conclusion instabilities unless there is a strong agreement among different methods. Therefore, in this paper, we evaluate the agreement between the feature importance ranks associated with the studied classifiers through a case study of 18 software projects and six commonly used classifiers. We find that: 1) The computed feature importance ranks by CA and CS methods do not always strongly agree with each other. 2) The computed feature importance ranks by the studied CA methods exhibit a strong agreement including the features reported at top-1 and top-3 ranks for a given dataset and classifier, while even the commonly used CS methods yield vastly different feature importance ranks. Such findings raise concerns about the stability of conclusions across replicated studies. We further observe that the commonly used defect datasets are rife with feature interactions and these feature interactions impact the computed feature importance ranks of the CS methods (not the CA methods). We demonstrate that removing these feature interactions, even with simple methods like CFS improves agreement between the computed feature importance ranks of CA and CS methods. In light of our findings, we provide guidelines for stakeholders and practitioners when performing model interpretation and directions for future research, e.g., future research is needed to investigate the impact of advanced feature interaction removal methods on computed feature importance ranks of different CS methods.

==> 06a-disc1.tex <==
\subsection{How discriminative are the top-3 reported features by the studied CS and CA methods?}

\label{sec:disc1}
\begin{figure*}
    \includegraphics[width=\linewidth,scale=1.5]{figures/disc_1_exp.pdf}
    \caption{Experiment setup of our discussion.}
    \label{fig:disc_1_exp_setup}
\end{figure*}

\textbf{Motivation: } From RQ1 (Section \ref{sec:rq1}), we observe that both CA and CS methods yield significantly different feature importance ranks on a given dataset for different classifiers. While such a result indicates that we cannot use one feature importance method in lieu of another, we do not know which of these feature importance methods yield the most discriminative (i.e., the features with the highest predictive capability) feature importance ranks. Such knowledge would help us with two things. First, to avoid the usage of a particular feature importance method that does not identify highly discriminative top-3 features (method filtering). Particularly, if any of the feature importance methods fail to identify highly discriminative features, we could discourage its usage. Second, to recommend the feature importance methods that could be more reliably used by researchers and practitioners (method recommendation). For instance, if one of the studied feature importance methods (amongst both CA and CS methods) consistently identifies the most discriminative top-3 feature set, we could recommend its usage over the other methods (even if all of these methods are highly discriminative).


\smallskip \noindent \textbf{Approach:} \textbf{Part 1 - Method filtering.} We present the experiment setup of our Discussion in Figure~\ref{fig:disc_1_exp_setup}. To estimate the discriminative capability of the top-3 computed features by each feature importance method, we first construct all of the studied classifiers using all the features of a given dataset as outlined in Section~\ref{subsec:classifier_construction}. Next, we construct classifiers with only the top-3 features given by the two CA methods, as well as the CS method of each classifier (please see Table~2 of Appendix~~B.3.1) for each studied dataset. We then measure the performance of the classifiers that are constructed using all the features against the performance of the classifiers that are constructed using the top-3 features. We measure the performance in terms of several performance measures (i.e., Accuracy, Precision, Recall, F1 Score, Brier Score and Mathew's Correlation Coefficient (MCC)) instead of using AUC as used in the earlier parts of our study. We do so in order to avoid the unfair advantage that the Permutation method would likely have, as such a method evaluates the importance of each feature based on their AUC performance (as outlined in Appendix~B.3.2). 
% of the classifier constructed on all the features and on the top-3 given by each of the studied feature importance method across all the studied performance measures
%We do so to observe whether the performance of a classifier constructed on all the features in a given dataset is significantly different with a large effect size from the performance of the classifier constructed on just the top-3 features generated by a given feature importance method.
Finally, we perform a Wilcoxon signed-rank test~\cite{wilcoxon1992individual} and a Cohen's d effect size difference test~\cite{cohen1992power} to compare the performance in a statistically rigorous manner. In the negative case (i.e., if the magnitude $\le 0.8$~\cite{cohen1992power}), we conclude that the performance of both classifiers is similar and thus the feature importance method is deemed as one that produces highly discriminative top-3 features. We consider a large Cohen's d effect size difference to quantify similarity over other cut-offs as we wanted to show that the differences in performances are large only if they differ by a considerable amount. If any of the studied feature importance methods fails to consistently produce highly discriminative top-3 features across the studied datasets, then we could discourage its use. 

\begin{table*}[!htbp]
  \centering
  \caption{No. of dataset on which classifiers that are constructed using the top 3 features given by the studied feature importance method has similar discriminative capability (i.e., if the Cohen's d $\le$ 0.8) as that of the classifier that is constructed using all the features of a dataset.}
\begin{threeparttable}
    \begin{tabular}{p{0.5cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}|p{0.2cm}p{0.2cm}p{0.2cm}}
    \hline
    \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Classifier}}} & \multicolumn{3}{c|}{\textbf{ACC}} & \multicolumn{3}{c|}{\textbf{PRE}} & \multicolumn{3}{c|}{\textbf{REC}} & \multicolumn{3}{c|}{\textbf{B-S}}  & \multicolumn{3}{c|}{\textbf{F-M}} & \multicolumn{3}{c}{\textbf{MCC}}\\
    
\cline{2-19}       & \textbf{CS} &\textbf{PD} & \textbf{PF} & \textbf{CS} & \textbf{PD} & \textbf{PF} & \textbf{CS} & \textbf{PD} & \textbf{PF} & \textbf{CS} & \textbf{PD} &\textbf{PF} & \textbf{CS} &\textbf{PD} & \textbf{PF} & \textbf{CS} & \textbf{PD} & \textbf{PF} \\
    \hline
    \multicolumn{1}{l|}{\textbf{glm}} &\multicolumn{1}{r}{16} &\multicolumn{1}{r}{14} &\multicolumn{1}{r|}{16} &\multicolumn{1}{r}{14} &\multicolumn{1}{r}{14} &\multicolumn{1}{r|}{14} &\multicolumn{1}{r}{10 } &\multicolumn{1}{r}{9} &\multicolumn{1}{r|}{10} &\multicolumn{1}{r}{9} &\multicolumn{1}{r}{7 } &\multicolumn{1}{r|}{8 }  &\multicolumn{1}{r}{10 } &\multicolumn{1}{r}{8 } &\multicolumn{1}{r|}{10} &\multicolumn{1}{r}{14} &\multicolumn{1}{r}{13} &\multicolumn{1}{r}{14} \\

    \multicolumn{1}{l|}{\textbf{rf}} &\multicolumn{1}{r}{5 } &\multicolumn{1}{r}{4 } &\multicolumn{1}{r|}{7 } &\multicolumn{1}{r}{6 } &\multicolumn{1}{r}{6 } &\multicolumn{1}{r|}{8 } &\multicolumn{1}{r}{8 } &\multicolumn{1}{r}{7 } &\multicolumn{1}{r|}{9 } &\multicolumn{1}{r}{5 } &\multicolumn{1}{r}{4 } &\multicolumn{1}{r|}{8 } &\multicolumn{1}{r}{3 } &\multicolumn{1}{r}{5 } &\multicolumn{1}{r|}{9 } &\multicolumn{1}{r}{4 } &\multicolumn{1}{r}{6 } &\multicolumn{1}{r}{7} \\

    \multicolumn{1}{l|}{\textbf{xgbTree}} &\multicolumn{1}{r}{10} &\multicolumn{1}{r}{8 } &\multicolumn{1}{r|}{8 } &\multicolumn{1}{r}{11} &\multicolumn{1}{r}{12} &\multicolumn{1}{r|}{9 } &\multicolumn{1}{r}{4 } &\multicolumn{1}{r}{3 } &\multicolumn{1}{r|}{4 } &\multicolumn{1}{r}{4 } &\multicolumn{1}{r}{0 } &\multicolumn{1}{r|}{1 }  &\multicolumn{1}{r}{5 } &\multicolumn{1}{r}{3 } &\multicolumn{1}{r|}{3 } &\multicolumn{1}{r}{10} &\multicolumn{1}{r}{9 } &\multicolumn{1}{r}{9} \\

    \multicolumn{1}{l|}{\textbf{rpart}} &\multicolumn{1}{r}{16} &\multicolumn{1}{r}{16} &\multicolumn{1}{r|}{16} &\multicolumn{1}{r}{16} &\multicolumn{1}{r}{16} &\multicolumn{1}{r|}{15} &\multicolumn{1}{r}{10} &\multicolumn{1}{r}{12} &\multicolumn{1}{r|}{11} &\multicolumn{1}{r}{7 } &\multicolumn{1}{r}{11} &\multicolumn{1}{r|}{9 }  &\multicolumn{1}{r}{10} &\multicolumn{1}{r}{12} &\multicolumn{1}{r|}{10} &\multicolumn{1}{r}{12} &\multicolumn{1}{r}{13} &\multicolumn{1}{r}{13} \\

    \multicolumn{1}{l|}{\textbf{C5.0Rules}} &\multicolumn{1}{r}{11} &\multicolumn{1}{r}{14} &\multicolumn{1}{r|}{13} &\multicolumn{1}{r}{9 } &\multicolumn{1}{r}{12} &\multicolumn{1}{r|}{12} &\multicolumn{1}{r}{4 } &\multicolumn{1}{r}{6 } &\multicolumn{1}{r|}{7 } &\multicolumn{1}{r}{8 } &\multicolumn{1}{r}{8 } &\multicolumn{1}{r|}{9 } &\multicolumn{1}{r}{4 } &\multicolumn{1}{r}{9 } &\multicolumn{1}{r|}{8 } &\multicolumn{1}{r}{13} &\multicolumn{1}{r}{14} &\multicolumn{1}{r}{13} \\

    \multicolumn{1}{l|}{\textbf{avNNet}} &\multicolumn{1}{r}{14} &\multicolumn{1}{r}{15} &\multicolumn{1}{r|}{15} &\multicolumn{1}{r}{15} &\multicolumn{1}{r}{12} &\multicolumn{1}{r|}{13} &\multicolumn{1}{r}{9 } &\multicolumn{1}{r}{12} &\multicolumn{1}{r|}{9 } &\multicolumn{1}{r}{7 } &\multicolumn{1}{r}{8 } &\multicolumn{1}{r|}{7 } &\multicolumn{1}{r}{10} &\multicolumn{1}{r}{11} &\multicolumn{1}{r|}{10} &\multicolumn{1}{r}{14} &\multicolumn{1}{r}{15} &\multicolumn{1}{r}{14}\\
    
    \hline
    \multicolumn{1}{l|}{\textbf{K-W (P-Val)}}  &\multicolumn{3}{c|}{\textbf{0.12}} &\multicolumn{3}{c|}{\textbf{0.89}} &\multicolumn{3}{c|}{\textbf{0.11}} &\multicolumn{3}{c|}{\textbf{0.65}}  &\multicolumn{3}{c|}{\textbf{0.19}} &\multicolumn{3}{c}{\textbf{0.24}}\\
    \hline

        \end{tabular}%
      \begin{tablenotes}
    \scriptsize
    \item 1. \textbf{Performance Measures:} ACC- Accuracy, PRE- Precision, REC- Recall, BS- Brier Score, F-M- F-Measure
    \item 2. \textbf{Feature importance methods:} CS- CS, PD- PDP, PF- Permutation  
    \item 3. \textbf{K-W} - Kruskal-Wallis H-Test P-Value 

\end{tablenotes}
\end{threeparttable}

  \label{tab:disc_table}%
\end{table*}%

\noindent \textbf{Part-2: Method recommendation.} To identify which of the studied feature importance methods can be recommended, for each dataset, we find the difference in performance between the classifiers that are constructed using all the features of the dataset and the classifiers that constructed only using the top-3 features given by the CA and CS methods - performance deltas (the smaller the difference, the higher the discriminative capability). Then to observe if any of the feature importance method consistently produces more discriminative features than the others, we rank the performance deltas. We do so on all the studied datasets for each classifier using the Scott-Knott ESD test (as shown in the first blue part of Figure~\ref{fig:disc_1_exp_setup}). Next, we aggregate the produced ranks on the performance deltas of the six studied classifiers across the three studied feature importance methods (2 CA methods and the studied CS method of the classifier) for all the 16 datasets (please refer the tables in Figure~\ref{fig:disc_1_exp_setup}) for each of the studied performance measure. For instance, for the Accuracy performance measure, we will have three distribution of ranks pertaining to the CS, PDP and Permutation CA methods. Each distribution will have six values corresponding (as given by the rank of the performance differences of the six studied classifiers) for each dataset (a total of 96 values per distribution). Each value in the distribution pertaining to a given feature importance method indicates its rank of discriminative capability in relation to the other feature importance methods on a given classifier and dataset. Finally, across each of the performance measure, we perform a paired Kruskal-Wallis H-test~\cite{kruskal1952use}. A p-value $\leq 0.05$ on the Kruskall-Wallis H-test between the rank distributions of CS, PDP and Permutation CA methods across all the performance measures would indicate that one of feature importance methods consistently yields more discriminative top-3 features than the other methods and we could recommend its usage. 
%\goliva{Ditto. This whole approach for 5.1 is still quite a bit convoluted. This is what I got from it after reading a few times (a) method filtering: check whether all features vs top-3 is statistically different with high effect size. If yes, then discard. Next we do (b) method recommendation. calculate the delta in the performance of all features vs top-3 for all classifiers on a dataset (how do you determine exactly perf difference? if I consider AUC, then is it median AUC on all features minus median AUC on top-3?) You'll have six values per FI method per dataset. Then for each dataset, I assume you run SK on the delta distributions to rank them. So for a dataset d1, you'll rank the FI methods into positions 1, 2 or 3. Then you do it for all datasets, so you end up with 16 rank lists I assume. Then you somehow aggregate these results and run Kruskal Wallis. This is what I understood and it's very complex. This part of the text needs to be way more digestible and I think that a simple yet nice diagram showing the key steps would help considerably. This is text writing issue essentially}

%For instance, consider the Eclipse-2.0 dataset and the random forest classifier. If the top 3 features given by PDP, Permutation and RFFI methods are (\texttt{pre, ACD, NOM\_avg}), (\texttt{ACD, NSF\_avg, PAR\_avg}) and (\texttt{pre, NBD\_avg, PAR\_avg}) respectively. Then we first build a random forest classifier with 100-out-of-sample bootstrap for the Eclipse-2.0 dataset with all the features and note down all the performance measures. Following which we build 3 separate random forest classifiers on (\texttt{pre, ACD, NOM\_avg}), (\texttt{NSF\_avg, PAR\_avg}) and (\texttt{pre, NBD\_avg, PAR\_avg}) with 100-out-of-sample bootstrap and note down the studied performance measures. We finally compute the difference in terms of all the performance measures between the random forest classifier constructed on top 3 features given by each of the feature importance method and the random forest classifier built on all the features of the Eclipse-2.0 dataset. The feature importance method that consistently yields the least difference in performance across all the studied performance measures could be considered to be the most discriminative. 


% Table generated by Excel2LaTeX from sheet 'Sheet1'
%\begin{table*}[htbp]
%  \centering
%  \caption{Add caption}
%    \begin{tabular}{l|r|r|r|r|r|r|}
%    \hline
%    \multicolumn{1}{c|}{\multirow{2}[4]{*}{\textbf{Dataset}}} & \multicolumn{2}{c|}{\textbf{CS}} & \multicolumn{2}{c|}{\textbf{PDP}} & \multicolumn{2}{c}{\textbf{Permutation}} \\
%\cline{2-7}    \multicolumn{1}{c|}{} & \multicolumn{1}{l|}{\textbf{p-value}} & \multicolumn{1}{l|}{\textbf{Cohen's d}} & \multicolumn{1}{l|}{\textbf{p-value}} & \multicolumn{1}{l|}{\textbf{Cohen's d}} & \multicolumn{1}{l|}{\textbf{p-value}} & \multicolumn{1}{l}{\textbf{Cohen's d}} \bigstrut\\
%    \hline
%    \textbf{Eclipse-2.0} & 0.1 & 0.12 (N) & 0.14 & 0.1 (N) & < 0 (S) & 0.67 (M)\\
%    \textbf{Eclipse-2.1} & 0.16 & -0.10 (N) & < 0 (S) & 0.36 (S) & < 0 (S) & 0.39 (S) \\
%    \textbf{Eclipse-3.0} & 0.38 & -0.02 (N) & < 0 (S) & 0.68 (M) & 0.54 & -0.01 (N) \\
%    \textbf{Eclipse34-debug} & \textbf{< 0 (S)} & \textbf{2.61 (L)} & < 0 (S) & -0.41 (S) & < 0 (S) & -0.43 (S) \\
%    \textbf{JM1} & < 0 (S) & 0.31 (S) & 0.39 & 0.02 (N) & 0.06 & -0.08 (N) \\
%    \textbf{Mylyn} & 0.58 & 0.03 (N) & 0.01 (S) & 0.25 (S) & 0.36 & 0.28 (S) \\
%    \textbf{PC5} & \textbf{< 0 (S)} & \textbf{3.38 (L)} & \textbf{< 0 (S)} & \textbf{2.26 (L)} & \textbf{< 0 (S)} & \textbf{1.43 (L)} \\
%    \textbf{PDE} & < 0 (S) & -0.73 (M) & < 0 (S) & -0.29 (S) & \textbf{< 0 (S)} & \textbf{-0.90 (L)} \\
%    \textbf{Poi-3.0} & 0.01 (S) & -0.28 (S) & 0.78 & 0.03 (N) & 0.74 & 0.04 (N) \\
%    \textbf{Prop-1} & \textbf{< 0 (S)} & \textbf{7.39 (L)} & \textbf{< 0 (S)} & \textbf{1.64 (L)} & \textbf{< 0 (S)} & \textbf{3.07 (L)} \\
%    \textbf{Prop-2} & < 0 (S) & 0.66 (M) & \textbf{< 0 (S)} & \textbf{8.44 (L)} & \textbf{< 0 (S)} & \textbf{1.67 (L)} \\
%    \textbf{Prop-3} & < 0 (S) & 0.55 (M) & \textbf{< 0 (S)} & \textbf{1.18 (L)} & \textbf{< 0 (S)} & \textbf{1.30 (L)} \\
%    \textbf{Prop-4} & < 0 (S) & 0.40 (M) & 0.26 & < 0 (N) & 0.01 (S) & 0.07 (N) \\
%    \textbf{Prop-5} & \textbf{< 0 (S)} & \textbf{6.55 (L)} & \textbf{< 0 (S)} & \textbf{2.47 (L)} & \textbf{< 0 (S)} & \textbf{1.89 (L)} \\
%    \textbf{Eclipse34-swt} & \textbf{< 0 (S)} & \textbf{1.82 (L)} & \textbf{< 0 (S)} & \textbf{1.09 (L)} & \textbf{< 0 (S)} & \textbf{1.80 (L)} \\
%    \textbf{Xalan-2.6} & < 0 (S) & -0.67 (M) & \textbf{< 0 (S)} & \textbf{-1.51 (L)} & 0.04 (S) & -0.22 (S) \\
 %   \hline
 %%   \end{tabular}%
%  \label{tab:disc2_tab1}%
%\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'

\smallskip \noindent \textbf{Results: Result 8) Method filtering:} \textbf{\textit{The top-3 most important features ascertained by all the studied feature importance methods are all highly discriminative}}. In Table~\ref{tab:disc_table}, we present the number of datasets on which the classifiers built using the top-3 features from each of the studied feature importance methods exhibits similar performances to the classifiers built using all the features. From Table~\ref{tab:disc_table} we observe that, all the studied feature importance methods exhibit similar capabilities in identifying the top 3 discriminative features for each of the studied classifiers across all the computed performance measures. For instance, consider the discriminative capability of the top-3 features given by the different methods in terms of Accuracy from Table~\ref{tab:disc_table}. Expect for the case of random forest and the xgbTree classifier, in at least 11 out of 16 datasets, the classifiers built using the top 3 features given by all the different feature importance methods, calculates Accuracy similar to that of the classifier built using all the features. Similar trends could be observed on all the threshold-dependent metrics like Precision, Recall, F-Measure and MCC. Each of classifier built using the top-3 features computed by the different feature importance methods exhibiting similar (high) discriminative capability indicates that each each feature importance method---though compute feature importances differently--- are a valid way of computing feature importances in their own right. 

The number of datasets on which the discriminative capability of the top-3 features being equivalent to that of all the features in a given dataset is lower in terms of the threshold-independent performance measure Brier Score. However, across the classifiers the different top-3 features computed by the different feature importance methods exhibit the similar characteristics even on threshold-independent measures. 



%Therefore, different feature importance methods producing different highly discriminative top 3 features indicate that there exist more than one unique subset of highly discriminative features in a given dataset. 

% We present the difference in AUC between the different classifiers constructed on all the features and the top 3 features given by each of the studied feature importance methods in Figure~\ref{fig:disc2_plot1}. From the Figure~\ref{fig:disc2_plot1} we observe that, the median difference in performance for almost all the studied datasets is within 15\% and the maximum performance difference is only within 20\%. Such narrow performance differences indicate that all the feature importance methods generate highly discriminative top 3 features. However, as we know from Section~\ref{sec:rqs}, we know that different feature importance methods generate different top 3 features.

\smallskip \noindent \textbf{Result 9) Method recommendation: \textit{No method consistently produces top-3 features with higher discriminative capability than other methods. Hence, we cannot recommend the use a particular feature importance method.}} We present the result of Kruskal-Wallis H-Test between the performance difference rank distributions of CS, PDP and Permutation CA methods in Table~\ref{tab:disc_table}. From the Table~\ref{tab:disc_table}, we observe that all the p-values are greater than 0.05. Such a result indicates that, across different performance measures, there is no one method that is consistently ranked low. Lack of clear separation in the discriminative capability of the top 3 features computed by different feature importance methods indicates that we cannot recommend usage of one of the feature importance method over another. 
%Particularly given that we know from Section~\ref{sec:rqs} that all the different feature importance methods yield different top 3 features with low Top 3 overlap among them.

%We present the results per classifier in Figure~\ref{fig:disc2_plot1}. A \textbf{low rank} for a given feature importance method signifies that the \textbf{top 3 features }generated by the particular method for the given classifier yields a performance that \textbf{closer to the performance of the same classifier} constructed on all the features. The Figure~\ref{fig:disc2_plot1} summarizes the results for each of the studied classifier across all the studied datasets and the performance measures.

%\begin{figure*}
%    \includegraphics[width=\linewidth,scale=1]{figures/disc2_rank_plots.pdf}

%    \caption{Rank of performance difference between classifier built on the top 3 features given by the feature importance method and the classifier built on the all the features of the dataset}
%    \label{fig:disc2_plot1}
%\end{figure*}


%\textbf{Among the studied classifiers, the studied feature importance methods excel in identifying the top 3 discriminative features of the decision tree classifier and struggle the most for random forest classifiers.}  For instance, we can observe that all the three studied feature importance methods identify the top 3 features that produce performance similar to that of that of the decision tree constructed on all the features of a dataset for 14 out of 16 datasets. Similarly, all the studied feature importance methods struggle to identify the most discriminative top 3 features of the random forest classifier. From Table~\ref{tab:disc_table} we see that only for 3 out of 16 datasets, the top 3 features identified by the feature importance methods yield a performance similar to that of the random forest built on all the features. Finally, we can also observe that characteristics of identifying the top 3 features is similar for all the other studied classifiers as evidenced from Table~\ref{tab:disc_table}.  %However, different methods ascertain different features to be the most important as we observe from Section~\ref{sec:rqs}). 


%\textbf{While all the studied feature importance methods yield highly discriminative top 3 features, the discriminativeness of the top 3 important features generated by the Permutation method is slightly higher than the other studied feature importance methods.} We rank the performance differences between the classifiers trained on the all the features and the top 3 features given by each of the feature importance method on the studied datasets with Scott-Knott ESD test. We present the results per classifier in Figure~\ref{fig:disc2_plot2}. A low rank for a given feature importance method signifies that the top 3 features generated by the particular method for the given classifier yields a performance that closer to the performance of the same classifier constructed on all the features. The Figure~\ref{fig:disc2_plot2} summarizes the results for each of the studied classifier across all the studied datasets. From the Figure, we observe that Permutation consistently has a median rank of 1 for 4 out of the 6 studied classifiers across all the studied datasets. Furthermore, the median rank given by the Permutation method consistently ranks between 1 to 2 for all the classifiers. However, CS and the PDP methods yield a median rank 1 only on 1 out of 6 classifiers and 2 out 6 classifiers across the datasets. Though all the studied feature importance methods yield highly discriminative top 3 features, Permutation generates slightly more discriminative features than the other studied feature importance methods. Therefore, we recommend the usage of Permutation method over the other studied feature importance computation methods. 

%\tastycolorbox{All of the studied feature importance methods produce top 3 features with similar discriminativeness despite producing different top 3 features, therefore it is impossible to recommend the usage of a particular feature importance method over another. }

%\gopi{I am not super sure if the following paragraph reads great, but I am not sure how to improve it. what do you think of it and any idea how to improve it?}
%\textbf{Such a small performance difference hints that there exist more than one unique subset of highly discriminative features and that none of the studied feature importance methods identify all the subsets.} We know from Section~\ref{sec:rqs} that the agreement and overlap between the feature importance ranks generated by the CS and CA (both within and across the) methods are low. However, from the experiments presented in this discussion, we find that (even on the same dataset and classifier) all the different sets of top 3 important features presented by both the CA and  CS methods are highly discriminative which shows that there are multiple unique subsets of highly discriminative features. Such a result hints that, different feature importance methods identify different subsets of highly discriminative features. Furthermore, these identified subsets depends more on how the feature importance method calculates the feature importance rather than what drives the classifier. For instance, consider LRFI and Permutation methods. The LRFI method ascertains feature importances by computing the t-statistic between the coefficient assigned to a feature and zero. The larger the t-statistic is, the higher the importance of that feature. However, this value captures how much a given feature reduces the defined internal loss of the classifier. Whereas in the case of Permutation, it takes a fitted classifier and ascertains how perturbation a given feature affects the performance of a classifier. While one method captures what affects the fit of the classifier, another method captures what affects the classifier's performance. While both of them seek to capture important properties of a classifier, both of them do not capture the whole picture and rather just captures how certain features affect the different aspects the feature importance methods are defined to capture. Because of which, each feature importance method captures different subset of top 3 important features. Because different methods yield different top 3 feature importance ranks and because no one method consistently produces more discriminative features than other methods, it is impossible to recommend usage of one feature importance method consistently even though all the feature importance methods yield highly discriminative features. 

%At this juncture, one could point out that, if all the feature importance methods yield highly discriminative features, we could simply use any of the feature importance methods to ascertain the feature importance ranks. However, in software engineering, researchers and practitioners typically use these feature importance ranks to formulate data-driven process improvements. From the results presented so far, we could observe that these feature importance methods only identify an aspect of what drives the model and that too based on what the feature importance computation method is designed to capture. In addition different feature importance computation methods yield different top 3 important features (see Section\ref{sec:rqs}). Therefore, using just any of the feature importance method to base the process improvements on could be potentially harmful. 

%Besides from just the discriminativeness of the features, the generalizability of feature importance ranks i.e., the feature importance  if we find that the top 3 features given by a classifier and feature importance method combination (e.g., random forest and PDP) consistently yields better performance on all the classifiers across the datasets than the top 3 features given by other feature importance methods (generalizability), we could recommend the usage of such combination to generate feature importance ranks. 
%Furthermore, from the results we could assert that, feature importance ranks generated by different feature importance methods depend on how the feature importance methods compute importance rather than what drives the classifier. We argue so because, as presented in Figure~\ref{fig:disc2_plot1}, the difference in performance between the classifiers built on all the features of a given dataset and the top 3 features given by all the studied feature importance methods is only within 2\%.


==> disc1_old.tex <==
\textbf{Can we recommend the usage of any particular FICM?}
\gopi{If we need space, I feel this discussion could go ..But Gustavo..Thoughts?}
\smallskip \noindent From Section~\ref{sec:rqs}, we observe that both CAFI and CSFI computation methods yield different feature importance ranks on a given dataset for different classifiers. While such results indicate that we cannot use one feature importance computation method in lieu of another for both CAFI and CSFI computation methods, we do not know which of these feature importance methods yield the most informative (i.e., the features with the highest predictive capability (in our case)) feature importance ranks. From Section~\ref{sec:related}, we observe that CSFI computation methods are more widely used by the software engineering community than CAFI methods as given by usages in~\cite{bird2011don,nagappan2006mining,tian2015characteristics,calefato2019empirical,fan2019impact,
jiarpakdee2019impact,rajbahadur2019impact,zimmermann2007predicting,gousios2014exploratory,
guo2004robust,kamei2012large}. Therefore, finding out which of the CSFI that yields the most informative feature importance ranks among the widely used CSFI computation methods would potentially allow us to recommend the usage of one of the studied CSFI computation methods to use.

To do so, on each of the studied datasets, we build all of the studied classifiers using only the features reported at the top 3 ranks given by each of the CSFI computation method. For instance, for the dataset Eclipse-2.0, consider that LRFI reports~\textit{loc, cbo} and \textit{dit} as the most important features. We then construct all the 6 studied classifiers using only~\textit{loc, cbo} and \textit{dit} as the independent features from Eclipse-2.0. As outlined in Section~\ref{sec:approach}, we perform a 100 out-of-sample bootstrap and measure the AUC for each iteration. We similarly construct all the 6 classifiers on the top 3 features reported by the CSFI computation method associated with each of the 6 classifiers for the Eclipse-2.0 dataset and note the performances. We repeat the similar procedure on all of the studied datasets and note down the 100-out-sample performances on each of the studied dataset for all the classifiers.

Once we have all the classifier's performance across the datasets, we check, for each of the constructed classifier, across the datasets, which of the CSFI copmutation method's top 3 features consistently yields the highest performance gains for a given classifier. We do so by first noting down the performance of each of the classifier, on the top 3 features given by the 6 CSFI computation methods. We then find the difference in performance between the classifier constructed on all the features and the same classifiers constructed on top 3 features given by the 6 CSFI computation methods. We do so for all the 6 studied classifiers. Following which, we rank the performance gains with Scott-Knott ESD. For instance, on Eclipse-2.0 dataset, we note down all the 100 out-of-sample performances of the logistic regression classifier on the top 3 features given by all the 6 CSFI computation methods. We then calculate the difference between the logistic regression classifier built on all the features and the logistic regression classifier built on the top 3 features given by all the 6 CSFI computation methods. Following which, we use the Scott-Knott ESD test and rank the performance gains to see which of the CSFI computation methods, resulted in generating the best performance for the logistic regression classifier. We repeat this procedure for all the 6 classifiers on all the studied datasets. Finally we observe, if across all the studied datasets, if any one CSFI computation method's top 3 features consistently yields the best performance gains on all the studied classifiers.

\begin{figure}
    \includegraphics[width=8cm,scale=1]{figures/Disc1_plot1.pdf}

    \caption{Performance ranks on all the six classifiers across the studied datasets given by top 3 features of the BFI computation methods.\gopi{to be polished}}
    \label{fig:Disc1_plot1}

\end{figure}

We find that none of the CSFI computation method's top 3 features consistently yield the best performance on all the classifiers across the datasets. We present the performance rankings achieved by the six studied classifiers across all the studied datasets when using different CSFI computation methods in Figure~\ref{fig:Disc1_plot1}. From Figure~\ref{fig:Disc1_plot1}, we observe that top 3 features from  RFFI, XGFI and NNFI achieve the achieve similar performance gains as indicated by a median rank of 2 for classifiers built on different top 3 features. Furthermore, the top three features given by LRFI, RFI and CRFI yields much lesser performance gains. Finally, we also observe that there is no one CSFI computation method that yields a consistently better performance across the classifiers. \textbf{Such a result indicates that none of the studied CSFI computation methods yield consistently more informative features than the others, while some CSFI methods like LRFI, RFI and CRFI encapsulate lesser information than the other CSFI computation methods.} This result, in addition with the results we observe from Section~\ref{sec:rqs} indicate that different CSFI computation methods yield different feature importance ranks and no one CSFI computation method consistently yields more informative feature importance ranks.

